In-medium polarization tensor in strong magnetic fields (I): Magneto-birefringence at finite temperature and density

We investigate in-medium polarization effects of the fermion and antifermion pairs at finite temperature and density in strong magnetic fields within the lowest Landau level approximation. Inspecting the integral representation of the polarization tensor by analytic and numerical methods, we provide both the real and imaginary parts of the polarization tensor obtained after delicate interplay between the vacuum and medium contributions essentially due to the Pauli-blocking effect. Especially, we provide a complete analytic form of the polarization tensor at zero temperature and finite density that exhibits an exact cancellation and associated relocation of the singular threshold behaviors for a single photon decay to a fermion and antifermion pair. As a physical application of the in-medium polarization tensor, we discuss the magneto-birefringence that is polarization-dependent dispersion relations of photons induced by the strong magnetic fields.

==> submission(I)-ver1/preamble.tex <==

%\usepackage[dvipdfmx]{graphicx,color}
%\usepackage[dvipdfmx]{graphicx}
\usepackage{graphicx}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{mathrsfs}
\usepackage{slashed}
\usepackage{ascmac}
\usepackage{comment}
%\usepackage{stix}
%\usepackage{wrapft}
%\usepackage{nidanfloat}

\usepackage{dcolumn}% Align table columns on decimal point

%\graphicspath{{../figs/}}

\allowdisplaybreaks[3]

%% Please include `dvipdfm' when you use dvi.
\usepackage[%dvipdfm, 
bookmarks=true,colorlinks,linkcolor=blue,urlcolor=cyan,citecolor=red]{hyperref}

%%%%%%%%%%%%%%%%%%%%%%%%

\def\dint{\int \hspace{-1.1em} - \, }
\renewcommand{\pl}{ {(+)} }
\newcommand{\mi}{ {(-)} }
\newcommand{\overlr}[1]{\overleftrightarrow{#1}}
\newcommand{\overl}[1]{\overleftarrow{#1}}
\newcommand{\overr}[1]{\overrightarrow{#1}}

\newcommand{\with}{\quad{\rm with}\quad}
\newcommand{\an}{\quad{\rm and}\quad}
\newcommand{\kin}{{\rm kin}}
\newcommand{\can}{{\rm can}}

\renewcommand{\cases}[1]{\left\{ \begin{array}{ll} #1 \end{array} \right. }
%\newcommand{\cout}[1]{ \begin{comment} {#1} \end{comment} }
\newcommand{\cout}[1]{ \if 0 {#1} \fi }
\newcommand{\Matrix}[1]{ \begin{pmatrix} #1 \end{pmatrix} }
\newcommand{\eqn}[1]{ \begin{eqnarray}  {#1} \end{eqnarray} }
\newcommand{\beq}{\begin{eqnarray}}
\newcommand{\eeq}{\end{eqnarray}}
\newcommand{\bseq}{\begin{subequations}}
\newcommand{\eseq}{\end{subequations}}
\newcommand{\nn}{\nonumber}
\renewcommand{\=}{&=&}
\newcommand{\nnb}{\nonumber \\}
\newcommand{\pd}{\partial}

\newcommand{\f}[2]{\frac{ {#1} }{ {#2} } }
\newcommand{\lr}[1]{\langle {#1} \rangle}
\newcommand{\LR}[1]{\left\langle {#1} \right\rangle}
\newcommand{\lan}{\langle} 
\newcommand{\ran}{\rangle}
\renewcommand{\l}{\left}
\renewcommand{\r}{\right}
\newcommand{\sbra}[1]{ { \left[ #1 \right] } }
\newcommand{\pare}[1]{ { \left\{ #1 \right\} } }

\newcommand\eref[1]{Eq.~(\ref{#1})}
\newcommand\fref[1]{Fig.~\ref{#1}}
\newcommand{\sla}{ \slashed }
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\abs}[1]{\left|#1\right|}

%%%%%%%%%% Greek alphabets
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\renewcommand{\d}{{\delta}}
\renewcommand{\k}{\kappa}
\renewcommand{\l}{\lambda}
\newcommand{\m}{\mu}
\newcommand{\n}{\nu}
\renewcommand{\r}{\rho}
\newcommand{\s}{\sigma}


\newcommand{\lam}{\lambda}
\newcommand{\Lam}{ \Lambda }


\newcommand{\ve}{\varepsilon}
\newcommand{\ep}{ \epsilon }
\newcommand{\vep}{ \varepsilon }
\newcommand{\Gam}{ \Gamma }
\newcommand{\gam}{ \gamma }
\newcommand{\bgam}{ {\bm \gamma} }

%%%%%%%%%% 3D vectors
\newcommand{\bx}{{\bm{x}}}
\newcommand{\by}{{\bm{y}}}
\newcommand{\bz}{{\bm{z}}}
\newcommand{\br}{{\bm{r}}}
\newcommand{\bk}{{\bm{k}}}
\newcommand{\bp}{{\bm{p}}}
\newcommand{\bq}{{\bm{q}}}
\newcommand{\bv}{{\bm{v}}}
\newcommand{\bA}{{\bm{A}}}
\newcommand{\bB}{{\bm B}}
\newcommand{\bE}{{\bm E}}
\newcommand{\bj}{{\bm j}}
\newcommand{\bsig}{{\bm \sigma}}
\newcommand{\bs}{{\bm s}}
\newcommand{\bn}{{\bm n}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bT}{\bm{T}}

\newcommand{\integ}{\int\!\!}
\newcommand{\xint}{\int d^4x}
\newcommand{\pint}{\int \frac{d^4p}{ (2\pi)^4}}
\newcommand{\tint}{\int_{-\infty}^{\infty}} 

\newcommand{\re}{\Re e}
\newcommand{\im}{\Im m}
%\newcommand{\arg}{{\rm arg}}
\newcommand{\id}{\mbox{1}\hspace{-0.25em}\mbox{l}}
\newcommand{\1}{\mbox{1}\hspace{-0.25em}\mbox{l}}


\newcommand{\A}{ {\mathcal A} }
\newcommand{\B}{ {\mathcal B} }
\newcommand{\C}{ {\mathcal C} }
\newcommand{\D}{ {\mathcal D} }
\newcommand{\E}{ {\mathcal E} }
\newcommand{\F}{ {\mathscr{F}} }
\newcommand{\G}{ {\mathscr{G}} }
\newcommand{\Ham}{ {\mathcal H} }

\newcommand{\K}{ {\mathcal K} }
\newcommand{\Lag}{ {\mathcal{L}} }
\newcommand{\M}{ {\mathcal M} }
\newcommand{\N}{ {\mathcal N} }
\newcommand{\order}{{\mathcal O}}
\newcommand{\prj}{ {\mathcal P} }
\newcommand{\Q}{ {\mathcal Q} }

\newcommand{\R}{ {\mathcal R} }
\newcommand{\T}{ {\mathcal T} }
\newcommand{\U}{ {\mathcal U} }
\newcommand{\V}{ {\mathcal V} }
\newcommand{\W}{ {\mathcal W} }
\newcommand{\X}{ {\mathcal X} }
\newcommand{\Y}{ {\mathcal Y } }
\newcommand{\Z}{ {\mathcal Z} }

\renewcommand{\Finv}{ {\mathscr{F}} }
\newcommand{\Ginv}{ {\mathscr{G}} }

\newcommand{\herc}{{\rm h.c.}}
\newcommand{\MeV}{ {\rm MeV} }
\newcommand{\GeV}{ {\rm GeV} }
\newcommand{\fm}{ {\rm fm} }
\newcommand{\as}{ \alpha_s }
\newcommand{\para}{ \parallel}
\newcommand{\tot}{ {\rm tot} }
\newcommand{\EM}{{\rm em}}
\newcommand{\Tr}{ {\rm Tr} }
\newcommand{\tr}{ {\rm tr} }
\newcommand{\diag}{ {\rm diag} }
\newcommand{\sgn}{ {\rm sgn} }
\newcommand{\ext}{ {\rm ext} }
\newcommand{\vac}{ {\rm vac} }
\newcommand{\Hall}{ {\rm Hall} }
\newcommand{\eff}{ {\rm eff} }
\newcommand{\fermion}{ {\rm fermion} }
\newcommand{\bson}{ {\rm boson} }
\newcommand{\quark}{ {\rm quark} }
\newcommand{\gluon}{ {\rm gluon} }
\newcommand{\ghost}{ {\rm ghost} }
\newcommand{\fin}{ {\rm fin} }
\renewcommand{\div}{ {\rm div} }
\newcommand{\UV}{ {\rm UV} }
\newcommand{\IR}{ {\rm IR} }
\newcommand{\NO}{ {\rm NO} }
\newcommand{\q}{ {\rm q} }
\newcommand{\YM}{ {\rm YM} }
\newcommand{\dyn}{ {\rm dyn} }
\newcommand{\LLL}{ {\rm LLL} }
\newcommand{\hLL}{ {\rm hLL} }
\newcommand{\QCD}{ {\rm QCD} }
\newcommand{\Res}{{ \rm Res }}
\newcommand{\Deb}{ {\rm Debye} }
\newcommand{\Li}{ {\rm  Li} }

\newcommand{\vp}{\vect{p}}
\newcommand{\vk}{\vect{k}}
\newcommand{\vl}{\vect{l}}
\newcommand{\vx}{\vect{x}}
\newcommand{\vgamma}{{\boldsymbol \gamma}}
\newcommand{\vzero}{\vect{0}}
\newcommand{\vv}{\vect{v}}
\newcommand{\vB}{\vect{B}}

\newcommand{\cond}{\kappa} %conductivity is \kappa or \sigma
\newcommand{\Bf}{B_f}
\newcommand{\qf}{q_f}
\newcommand{\Tc}{{\mathrm T}_C}
\newcommand{\Nc}{N_c}
\newcommand{\Nf}{N_f}
\newcommand{\nf}{n_F}
\newcommand{\nb}{n_B}
\newcommand{\eL}{\epsilon^L}
\newcommand{\Cf}{C_f}

\newcommand{\zero}{{(0)}}
\newcommand{\one}{{(1)}}
\newcommand{\two}{{(2)}}

\newcommand{\matt}{{\rm matt}}

%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tilU}{\widetilde{U}}
\newcommand{\tilA}{\widetilde{A}}
\newcommand{\tilD}{\widetilde{D}}
\newcommand{\tilScal}{\widetilde{\mathcal{S}}}
\newcommand{\tilHcal}{\widetilde{\mathcal{H}}}
\newcommand{\hSigma}{\hat{\Sigma}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hpi}{\hat{\pi}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hTheta}{\hat{\Theta}}
\newcommand{\hlam}{\hat{\lambda}}
\newcommand{\hbeta}{\hat{\beta}}
\newcommand{\hM}{\hat{M}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hD}{\hat{D}}
\newcommand{\Hcal}{\mathcal{H}}

\newcommand{\tile}{\tilde{e}}
\newcommand{\tilg}{\tilde{g}}
\newcommand{\tilt}{\tilde{t}}
\newcommand{\tilb}{\tilde{b}}
\newcommand{\tilx}{\tilde{x}}
\newcommand{\tily}{\tilde{y}}
\newcommand{\tils}{\tilde{s}}
\newcommand{\tilN}{\tilde{N}}
\newcommand{\tilB}{\tilde{B}}
\newcommand{\tilOcal}{\tilde{\mathcal{O}}}
\newcommand{\tiln}{\tilde{n}}
\newcommand{\tilu}{\tilde{u}}
\newcommand{\tilj}{\tilde{j}}
\newcommand{\tildelta}{\tilde{\delta}}
\newcommand{\tilpartial}{\tilde{\partial}}
\newcommand{\tilF}{\widetilde{F}}
\newcommand{\tilh}{\tilde{h}}

\newcommand{\diff}{\mathrm{d}}
\newcommand{\average}[1]{\langle#1\rangle}
\newcommand{\baverage}[1]{\Big\langle#1\Big\rangle}
\newcommand{\baverageLG}[1]{\Big\langle#1\Big\rangle^{\mathrm{LG}}}

\newcommand{\hT}{\hat{T}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\hc}{\hat{c}}
\newcommand{\hS}{\hat{S}}
\newcommand{\hs}{\hat{s}}
\newcommand{\hP}{\hat{P}}
\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hPhi}{\hat{\Phi}}
\newcommand{\hU}{\hat{U}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{color} % For blue in-text comments and additions
\usepackage[normalem]{ulem}  % \sout{old text} for strikeout
%\renewcommand\sout{\bgroup \color{red} \ULdepth=-.5ex \ULset}
\newcommand{\com}[1]{[{\color[rgb]{0,0,1}{#1}}]}
\newcommand{\modi}[1]{{\color[rgb]{0,0,1}{#1}}}
\newcommand{\cgd}[1]{{\color[rgb]{1,0,0}{#1}}}
\newcommand{\changed}[1]{{\color[rgb]{1,0,0}{#1}}}
\newcommand{\gray}[1]{{\color[rgb]{0.7,0.7,0.7}{#1}}}
\newcommand{\gr}[1]{{\color[rgb]{0.3,0.6,0.3}{#1}}}
\newcommand{\blue}[1]{{\color[rgb]{0.2,0.6,0.9}{#1}}}
\newcommand{\red}[1]{{\color[rgb]{0.9,0.2,0.6}{#1}}}
\newcommand{\pp}[1]{{\color[rgb]{0.7,0.3,0.9}{#1}}}
\newcommand{\bro}[1]{{\color[rgb]{0.5,0.3,0.3}{#1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
